KiDS-1000 Cosmology: Multi-probe weak gravitational lensing and spectroscopic galaxy clustering constraints

We present a joint cosmological analysis of weak gravitational lensing observations from the Kilo-Degree Survey (KiDS-1000), with redshift-space galaxy clustering observations from the Baryon Oscillation Spectroscopic Survey (BOSS), and galaxy-galaxy lensing observations from the overlap between KiDS-1000, BOSS and the spectroscopic 2-degree Field Lensing Survey (2dFLenS). This combination of large-scale structure probes breaks the degeneracies between cosmological parameters for individual observables, resulting in a constraint on the structure growth parameter $S_8=\sigma_8 \sqrt{\Omega_{\rm m}/0.3} = 0.766^{+0.020}_{-0.014}$, that has the same overall precision as that reported by the full-sky cosmic microwave background observations from Planck. The recovered $S_8$ amplitude is low, however, by $8.3 \pm 2.6$ % relative to Planck. This result builds from a series of KiDS-1000 analyses where we validate our methodology with variable depth mock galaxy surveys, our lensing calibration with image simulations and null-tests, and our optical-to-near-infrared redshift calibration with multi-band mock catalogues and a spectroscopic-photometric clustering analysis. The systematic uncertainties identified by these analyses are folded through as nuisance parameters in our cosmological analysis. Inspecting the offset between the marginalised posterior distributions, we find that the $S_8$-difference with Planck is driven by a tension in the matter fluctuation amplitude parameter, $\sigma_8$. We quantify the level of agreement between the CMB and our large-scale structure constraints using a series of different metrics, finding differences with a significance ranging between $\sim\! 3\,\sigma$, when considering the offset in $S_{8}$, and $\sim\! 2\,\sigma$, when considering the full multi-dimensional parameter space.

==> blindBandC.tex <==

\begin{figure}
	\begin{center}
		\includegraphics[width=\columnwidth]{Parameter_Plots/cosmology/omegam_sigma8_h_blind_B}
		\caption{Constraints on flat $\Lambda$CDM blind B}
		\label{fig:cosmology-paramsB}
	\end{center}
\end{figure}

\begin{figure}
	\begin{center}
		\includegraphics[width=\columnwidth]{Parameter_Plots/cosmology/omegam_sigma8_h_blind_C}
		\caption{Constraints on flat $\Lambda$CDM blind C}
		\label{fig:cosmology-paramsC}
	\end{center}
\end{figure}


\begin{figure}
	\begin{center}
		\includegraphics[width=\columnwidth]{Parameter_Plots/systematics/S8_comparison_blindB}
		\caption{Constraints on $S_{8}$ blind B}
		\label{fig:S8compB}
	\end{center}
\end{figure}

\begin{figure}
	\begin{center}
		\includegraphics[width=\columnwidth]{Parameter_Plots/systematics/S8_comparison_blindA}
		\caption{Constraints on $S_{8}$ blind A}
		\label{fig:S8compA}
	\end{center}
\end{figure}


\begin{figure*}
	\begin{center}
		\includegraphics[width=\textwidth]{Parameter_Plots/cosmology/omegam_sigma8_s8_ns_h_a_baryon_a_ia_b1l_b1h_blind_B}
		\caption{Constraints blind B}
		\label{fig:cosmology-params-allB}
	\end{center}
\end{figure*}

\begin{figure*}
	\begin{center}
		\includegraphics[width=\textwidth]{Parameter_Plots/cosmology/omegam_sigma8_s8_ns_h_a_baryon_a_ia_b1l_b1h_blind_C}
		\caption{Constraints blind C}
		\label{fig:cosmology-params-allC}
	\end{center}
\end{figure*}

\begin{table}
	\begin{center}
		\caption{Goodness of fit for blind B}
		\label{tab:goodness-of-fitB}
\begin{tabular}{lrcl}
    \toprule
    Probe             & $\chi^2$       & DoF       & $p$-value   \\
    \midrule
	CS               & $< 151.3$ & $120-4.5$ & 0.014 \\
	GC               & $< 169.5$ & $168-13$ & 0.202 \\
	CS+GGL           & $176.1$ & $142-7$ & 0.010 \\
	3x2pt            & $353.0$ & $310-20$ & 0.007 \\

    \bottomrule
\end{tabular}
	\end{center}
\end{table}

\begin{table}
	\begin{center}
		\caption{Goodness of fit for blind C}
		\label{tab:goodness-of-fitC}
\begin{tabular}{lrcl}
    \toprule
    Probe             & $\chi^2$       & DoF       & $p$-value   \\
    \midrule
	CS               & $< 150.8$ & $120-4.5$ & 0.015 \\
	GC               & $< 169.5$ & $168-13$ & 0.202 \\
	CS+GGL           & $< 178.5$ & $142-7$ & 0.007 \\
	3x2pt            & $352.9$ & $310-20$ & 0.007 \\

    \bottomrule
\end{tabular}
	\end{center}
\end{table}

